Semantic Style Transfer for Enhancing Animal Facial Landmark Detection

Neural Style Transfer (NST) is a technique for applying the visual characteristics of one image onto another while preserving structural content. Traditionally used for artistic transformations, NST has recently been adapted, e.g., for domain adaptation and data augmentation. This study investigates the use of this technique for enhancing animal facial landmark detectors training. As a case study, we use a recently introduced Ensemble Landmark Detector for 48 anatomical cat facial landmarks and the CatFLW dataset it was trained on, making three main contributions. First, we demonstrate that applying style transfer to cropped facial images rather than full-body images enhances structural consistency, improving the quality of generated images. Secondly, replacing training images with style-transferred versions raised challenges of annotation misalignment, but Supervised Style Transfer (SST) - which selects style sources based on landmark accuracy - retained up to 98% of baseline accuracy. Finally, augmenting the dataset with style-transferred images further improved robustness, outperforming traditional augmentation methods. These findings establish semantic style transfer as an effective augmentation strategy for enhancing the performance of facial landmark detection models for animals and beyond. While this study focuses on cat facial landmarks, the proposed method can be generalized to other species and landmark detection models.

==> anadilSections/relatedwork.tex <==
\section{background}
\label{sec:background}
Affective computing in cats focuses on analyzing facial and behavioral cues to infer emotional states such as pain and stress. Traditional assessment methods, including the Feline Grimace Scale (FGS), rely on manual scoring, which is subjective and requires expert training \cite{evangelista2019facial}. To address these limitations, automated deep learning models have been introduced, improving accuracy and scalability in feline emotion recognition.

Feighelstein et al. \cite{feighel} explored AI-driven pain detection in domestic short-haired cats, evaluating two approaches: a CNN-based model (ResNet50) for analyzing facial images and a geometric facial landmark-based model inspired by the Cat Facial Action Coding System (CatFACS). Both methods demonstrated over 72\% accuracy, reinforcing the feasibility of automated pain assessment in felines \cite{Feighelstein2022}. Further studies emphasized the importance of explainability in AI models, ensuring transparency in veterinary applications \cite{Feighelstein2023}.

Facial landmark detection plays a fundamental role in feline affective computing, offering a structured approach to analyzing expressions. The Cat Facial Landmarks in the Wild (CatFLW) dataset introduced a standardized benchmark for training and evaluating deep learning models, comprising 2,000+ images annotated with 48 anatomical landmarks \cite{Martvel2023CatFLW}. Martvel et al. \cite{Martvel2024Detection} extended this work by developing a CNN-based landmark detector utilizing a magnifying ensemble method, significantly improving detection accuracy. This model has since been applied to broader applications, including breed classification, cephalic type identification, and pain detection, achieving 75\% accuracy in cephalic type classification and 66\% accuracy in pain assessment \cite{Martvel2024Analysis}.

Recent advancements have integrated YOLOv8-based face detection with an Ensemble Landmark Detector (ELD), enabling video-based pain assessment \cite{Martvel2024Video}. Additionally, novel architectures such as Siamese Comparative Transformer-based Networks (SCTN) have been introduced to enhance unsupervised landmark detection, demonstrating exceptional performance in extracting meaningful facial landmarks \cite{Martvel2024Video}.

Neural Style Transfer (NST) was initially introduced as a technique for artistic image transformation, enabling the fusion of image content and stylistic elements \cite{v1Gayts2015ArtisticStyle}. Over time, NST has been adapted for applications such as domain adaptation, image-to-image translation, and dataset augmentation \cite{v1JohnsonSuperResoluation2016, a_Li2017, a_Ledig2017}. The core concept involves extracting content features and style attributes using deep neural networks, recombining them to generate a stylized image while preserving structural integrity \cite{Huang2017, deepPhST}.

Traditional NST relied on CNN-based transformations, which were later extended through Generative Adversarial Networks (GANs). Methods such as Pix2Pix \cite{Pix2PixIsola2018} and CycleGAN \cite{CycleGAN_img2img} enabled more flexible image-to-image translation without requiring paired datasets. While these methods significantly enhanced style transfer realism, they often introduced geometric distortions, making them unsuitable for structured data such as facial images \cite{Structure-PreservingCheng2019}.

To address these issues, semantic-aware models were developed to ensure that style transformations respect spatial structures \cite{Liao2017}. Unlike traditional NST and GAN-based techniques, semantic style transfer allows localized style modifications that correspond to key facial regions, improving control over structural consistency \cite{Hong2021}.

More recently, Vision Transformers (ViTs) have introduced a new paradigm in style transfer by leveraging self-attention mechanisms to capture long-range dependencies in an image \cite{dosovitskiy2020vit}. Among these, Splice ViT has demonstrated strong performance in semantic visual appearance transfer, ensuring that style modifications do not disrupt structural coherence \cite{Tumanyan2022SpliceViT}. Unlike GAN-based models, Splice ViT encodes content and style separately, allowing for precise transformations that retain essential spatial features.

Although these advancements have improved realism and structural integrity in NST-generated images, challenges remain in applying style transfer for data augmentation in animal imagery. One of the primary concerns is ensuring that style transformations maintain anatomical accuracy, as distortions could negatively impact model predictions. Additionally, computational efficiency is a challenge, given that transformer-based methods require substantial processing resources. Lastly, semantic alignment must be carefully managed to ensure that stylistic modifications do not introduce unintended distortions in key facial features.

Building on these advancements, this study explores the application of Splice ViT for enhancing training datasets in cat facial landmark detection, evaluating its impact on model performance and structural consistency.
